Antennas for the Detection of Radio Emission Pulses from Cosmic-Ray induced Air Showers at the Pierre Auger Observatory

The Pierre Auger Observatory is exploring the potential of the radio detection technique to study extensive air showers induced by ultra-high energy cosmic rays. The Auger Engineering Radio Array (AERA) addresses both technological and scientific aspects of the radio technique. A first phase of AERA has been operating since September 2010 with detector stations observing radio signals at frequencies between 30 and 80 MHz. In this paper we present comparative studies to identify and optimize the antenna design for the final configuration of AERA consisting of 160 individual radio detector stations. The transient nature of the air shower signal requires a detailed description of the antenna sensor. As the ultra-wideband reception of pulses is not widely discussed in antenna literature, we review the relevant antenna characteristics and enhance theoretical considerations towards the impulse response of antennas including polarization effects and multiple signal reflections. On the basis of the vector effective length we study the transient response characteristics of three candidate antennas in the time domain. Observing the variation of the continuous galactic background intensity we rank the antennas with respect to the noise level added to the galactic signal.

==> TitlePage.tex <==
  \begin{titlepage}
    
    \title{Antennas for the Detection of Radio Emission Pulses from Cosmic-Ray induced Air Showers at the Pierre Auger Obervatory}
    \maketitle

%     \author[PA,PA2]{The Pierre Auger Collaboration}
%     \author[SUB]{Didier Charrier}
%     \author[NAN]{Laurent Denis}
%     \author[RWTH]{G\"unter Hilgers}
%     \author[KIT]{Oliver Kr\"omer}
%     \author[RWTH]{Lars Mohrmann}
%     \author[RWTH]{Barthel Philipps}
%     \author[RWTH]{Oliver Seeger}
%     \address[PA]{Av. San Mart\'in Norte 304 (5613) Malarg\"ue, Prov. de Mendoza, Argentina}
%     \address[PA2]{A full author list and affiliations can be found at http://www.auger.org/authors.html}
%     \address[SUB]{SUBATECH, \'{E}cole des Mines de Nantes, CNRS-IN2P3, Universit\'{e} de Nantes, Nantes, France}
%     \address[NAN]{Station de Radioastronomie de Nan\c{c}ay, Observatoire de Paris, Nan\c{c}ay, France}
%     \address[RWTH]{RWTH Aachen University, III. Physikalisches Institut A, Aachen, Germany}
%     \address[KIT]{Karlsruhe Institute of Technology - Campus North - Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
      
    \input{author_list_latex2}
    
    
    \begin{abstract}
      The Pierre Auger Observatory is exploring the potential of the radio detection technique to study extensive air showers induced by ultra-high energy cosmic rays.
%       within the surface detector of its observatory. 
      The Auger Engineering Radio Array (AERA) addresses both technological and scientific aspects of the radio technique. A first phase of AERA has been operating since September 2010 with detector stations observing radio signals at frequencies between 30 and 80 MHz. In this paper we present comparative studies to identify and optimize the antenna design for the final configuration of AERA consisting of 160 individual radio detector stations. 
      The transient nature of the air shower signal requires a detailed description of the antenna sensor.
      As the ultra-wideband reception of pulses is not widely discussed in antenna literature,
      we review the relevant antenna characteristics and enhance theoretical considerations towards the impulse response of antennas including polarization effects and multiple signal reflections.
%       new double sentence:
      On the basis of the vector effective length we study the transient response characteristics of three candidate antennas in the time domain. 
      Observing the variation of the continuous galactic background intensity we rank the antennas with respect to the noise level added to the galactic signal.
%       Observing the variation of the continuous galactic background intensity we discriminate the antennas with respect to an optimal noise performance.
%       old single sentence:
%       Observing the variation of the continuous galactic background intensity we discriminate candidate antennas with respect to an optimal noise performance.
      
    \end{abstract}
%     \begin{keyword}
      % keywords here, in the form: keyword \sep keyword
%       Cosmic Rays \sep Air Showers \sep Radio Detection \sep Antennas \sep AERA \sep Pierre Auger Observatory
%     \end{keyword}
%     \global\let\newpagegood\newpage
%     \global\let\newpage\relax
%     \let\endtitlepage\relax

    \end{titlepage}
    
  % restore the \newpage command after creating the title page
%   \global\let\newpage\newpagegood


==> TitlePage2.tex <==
 \vfill \begin{center} {\Large 
Antennas for the Detection of Radio Emission Pulses from Cosmic-Ray induced Air Showers at the Pierre Auger Obervatory
\par}
\vskip0.5cm
\end{center}
\input{author_list_latex2}
\twocolumn
% \begin{abstract*}[tp]
\twocolumn[
  \begin{@twocolumnfalse}

\noindent\hrulefill
  \vskip0.15cm
  \noindent \textbf{Abstract}
  \vskip0.15cm
  \noindent The Pierre Auger Observatory is exploring the potential of the radio detection technique to study extensive air showers induced by ultra-high energy cosmic rays.
  %       within the surface detector of its observatory. 
  The Auger Engineering Radio Array (AERA) addresses both technological and scientific aspects of the radio technique. A first phase of AERA has been operating since September 2010 with detector stations observing radio signals at frequencies between 30 and 80 MHz. In this paper we present comparative studies to identify and optimize the antenna design for the final configuration of AERA consisting of 160 individual radio detector stations. 
  The transient nature of the air shower signal requires a detailed description of the antenna sensor.
  As the ultra-wideband reception of pulses is not widely discussed in antenna literature,
  we review the relevant antenna characteristics and enhance theoretical considerations towards the impulse response of antennas including polarization effects and multiple signal reflections.
  %       new double sentence:
  On the basis of the vector effective length we study the transient response characteristics of three candidate antennas in the time domain. 
  Observing the variation of the continuous galactic background intensity we rank the antennas with respect to the noise level added to the galactic signal.
  %       Observing the variation of the continuous galactic background intensity we discriminate the antennas with respect to an optimal noise performance.
  %       old single sentence:
  %       Observing the variation of the continuous galactic background intensity we discriminate candidate antennas with respect to an optimal noise performance.
% \hline    

  \noindent\hrulefill
  \end{@twocolumnfalse}
  \vskip0.30cm
]

% \end{abstract*}


==> author_list_latex.tex <==
% This is a fragment that can be inserted into a LaTeX
% \par\noinde
% {\bf The Pierre Auger Collaboration} \\
\author[65]{P.~Abreu}
\author[53]{M.~Aglietta}
\author[95]{M.~Ahlers}
\author[83]{E.J.~Ahn}
\author[16]{I.F.M.~Albuquerque}
\author[30]{D.~Allard}
\author[1]{I.~Allekotte}
\author[87]{J.~Allen}
\author[89]{P.~Allison}
\author[11,7]{A.~Almela}
\author[58]{J.~Alvarez Castillo}
\author[75]{J.~Alvarez-Mu\~{n}iz}
\author[17]{R.~AlvesBatista}
\author[47]{M.~Ambrosio}
\author[59]{A.~Aminaei}
\author[96]{L.~Anchordoqui}
\author[65]{S.~Andringa}
\author[24]{T.~Anti\v{c}i'{c}}
\author[47]{C.~Aramo}
\author[4,72]{E.~Arganda}
\author[72]{F.~Arqueros}
\author[1]{H.~Asorey}
\author[65]{P.~Assis}
\author[32]{J.~Aublin}
\author[38]{M.~Ave}
\author[33]{M.~Avenier}
\author[10]{G.~Avila}
\author[42]{T.~B\"{a}cker}
\author[68]{A.M.~Badescu}
\author[37]{M.~Balzer}
\author[12]{K.B.~Barber}
% \author[14~‡]{A.F.~Barbosa}
\author[31]{R.~Bardenet}
\author[19]{S.L.C.~Barroso}
% \author[89~f]{B.~Baughman}
\author[36]{J.~B\"{a}uml}
\author[89]{J.J.~Beatty}
\author[94]{B.R.~Becker}
\author[35]{K.H.~Becker}
\author[34]{A.~Bell\'{e}toile}
\author[12]{J.A.~Bellido}
\author[95]{S.~BenZvi}
\author[33]{C.~Berat}
\author[1]{X.~Bertou}
\author[39]{P.L.~Biermann}
\author[32]{P.~Billoir}
\author[72]{F.~Blanco}
\author[32,73]{M.~Blanco}
\author[35]{C.~Bleve}
\author[38,36]{H.~Bl\"{u}mer}
\author[26]{M.~Boh\'{a}\v{c}ov\'{a}}
\author[48]{D.~Boncioli}
\author[22,32]{C.~Bonifazi}
\author[53]{R.~Bonino}
\author[63]{N.~Borodai}
\author[81]{J.~Brack}
\author[66]{I.~Brancus}
\author[65]{P.~Brogueira}
\author[82]{W.C.~Brown}
% \author[77~i]{R.~Bruijn}
\author[42]{P.~Buchholz}
\author[74]{A.~Bueno}
\author[79]{R.E.~Burton}
\author[90]{K.S.~Caballero-Mora}
\author[45]{B.~Caccianiga}
\author[39]{L.~Caramete}
\author[49]{R.~Caruso}
\author[53]{A.~Castellina}
\author[52]{O.~Catalano}
\author[46]{G.~Cataldi}
\author[65]{L.~Cazon}
\author[50]{R.~Cester}
\author[33]{J.~Chauvin}
\author[90]{S.H.~Cheng}
\author[53]{A.~Chiavassa}
\author[17]{J.A.~Chinellato}
\author[86]{J.~Chirinos Diaz}
\author[26]{J.~Chudoba}
\author[47]{M.~Cilmo}
\author[12]{R.W.~Clay}
\author[46]{M.R.~Coluccia}
\author[65]{R.~Concei\c{c}\~{a}o}
\author[9]{F.~Contreras}
\author[77]{H.~Cook}
\author[12]{M.J.~Cooper}
\author[59,61]{J.~Coppens}
\author[31]{A.~Cordier}
\author[90]{S.~Coutu}
\author[79]{C.E.~Covault}
\author[30]{A.~Creusot}
\author[90]{A.~Criss}
\author[92]{J.~Cronin}
\author[39]{A.~Curutiu}
\author[31]{S.~Dagoret-Campagne}
\author[34]{R.~Dallier}
\author[17]{B.~Daniel}
\author[5,3]{S.~Dasso}
\author[36]{K.~Daumiller}
\author[12]{B.R.~Dawson}
\author[23]{R.M.~de Almeida}
\author[49]{M.~De Domenico}
\author[58]{C.~De Donato}
\author[59,61]{S.J.~de Jong}
\author[8]{G.~De La Vega}
\author[17]{W.J.M.~de Mello Junior}
\author[22]{J.R.T.~de Mello Neto}
\author[46]{I.~De Mitri}
\author[15]{V.~de Souza}
\author[60]{K.D.~de Vries}
\author[73]{L.~del Peral}
\author[48,9]{M.~del R\'{\i}o}
\author[29]{O.~Deligny}
\author[38]{H.~Dembinski}
\author[86]{N.~Dhital}
\author[48,44]{C.~DiGiulio}
\author[14]{M.L.~D\'{\i}azCastro}
\author[97]{P.N.~Diep}
\author[65]{F.~Diogo}
\author[17]{C.~Dobrigkeit}
\author[60]{W.~Docters}
\author[58]{J.C.~D'Olivo}
\author[97,29]{P.N.~Dong}
\author[81]{A.~Dorofeev}
\author[14]{J.C.~dos Anjos}
\author[4]{M.T.~Dova}
\author[47]{D.~D'Urso}
\author[39]{I.~Dutan}
\author[26]{J.~Ebr}
\author[36]{R.~Engel}
\author[40]{M.~Erdmann}
\author[83,17]{C.O.~Escobar}
\author[65]{J.~Espadanal}
\author[7,11]{A.~Etchegoyen}
\author[92]{P.~FacalSanLuis}
\author[59,62]{H.~Falcke}
\author[87]{G.~Farrar}
\author[17]{A.C.~Fauth}
\author[83]{N.~Fazzini}
\author[79]{A.P.~Ferguson}
\author[86]{B.~Fick}
\author[7]{A.~Filevich}
\author[69,70]{A.~Filip\v{c}i\v{c}}
\author[40]{S.~Fliescher}
\author[81]{C.E.~Fracchiolla}
\author[60]{E.D.~Fraenkel}
\author[68]{O.~Fratu}
\author[42]{U.~Fr\"{o}hlich}
\author[38]{B.~Fuchs}
\author[32]{R.~Gaior}
\author[7]{R.F.~Gamarra}
\author[43]{S.~Gambetta}
\author[8]{B.~Garc\'{\i}a}
\author[75]{S.T.~GarciaRoca}
\author[31]{D.~Garcia-Gamez}
\author[72]{D.~Garcia-Pinto}
\author[74]{A.~Gascon Bravo}
\author[37]{H.~Gemmeke}
\author[32]{P.L.~Ghia}
\author[64]{M.~Giller}
\author[8]{J.~Gitto}
\author[83]{H.~Glass}
\author[94]{M.S.~Gold}
\author[1]{G.~Golup}
\author[4]{F.~Gomez Albarracin}
\author[1]{M.~G\'{o}mez Berisso}
\author[10]{P.F.~G\'{o}mez Vitale}
\author[65]{P.~Gon\c{c}alves}
\author[36]{J.G.~Gonzalez}
\author[81]{B.~Gookin}
\author[53]{A.~Gorgi}
\author[16]{P.~Gouffon}
\author[89]{E.~Grashorn}
\author[59,61]{S.~Grebe}
\author[89]{N.~Griffith}
\author[40]{M.~Grigat}
\author[54]{A.F.~Grillo}
\author[3]{Y.~Guardincerri}
\author[47]{F.~Guarino}
\author[18]{G.P.~Guedes}
\author[4]{P.~Hansen}
\author[1]{D.~Harari}
\author[12]{T.A.~Harrison}
\author[81]{J.L.~Harton}
\author[36]{A.~Haungs}
\author[40]{T.~Hebbeker}
\author[36]{D.~Heck}
\author[12]{A.E.~Herve}
\author[83]{C.~Hojvat}
\author[92]{N.~Hollon}
\author[12]{V.C.~Holmes}
\author[63]{P.~Homola}
\author[59]{J.R.~H\"{o}randel}
\author[27]{P.~Horvath}
\author[27,26]{M.~Hrabovsk\'{y}}
\author[38]{D.~Huber}
\author[36]{T.~Huege}
\author[49]{A.~Insolia}
\author[92]{F.~Ionita}
\author[49]{A.~Italiano}
\author[4]{C.~Jarne}
\author[59]{S.~Jiraskova}
\author[7]{M.~Josebachuili}
\author[24]{K.~Kadija}
\author[35]{K.H.~Kampert}
\author[25]{P.~Karhan}
\author[83]{P.~Kasper}
\author[38]{I.~Katkov}
\author[31]{B.~K\'{e}gl}
\author[36]{B.~Keilhauer}
\author[85]{A.~Keivani}
\author[59]{J.L.~Kelley}
\author[17]{E.~Kemp}
\author[86]{R.M.~Kieckhafer}
\author[36]{H.O.~Klages}
\author[37]{M.~Kleifges}
\author[9,36]{J.~Kleinfeller}
\author[77]{J.~Knapp}
\author[33]{D.-H.~Koang}
\author[92]{K.~Kotera}
\author[35]{N.~Krohm}
\author[37]{O.~Kr\"{o}mer}
\author[35]{D.~Kruppke-Hansen}
\author[83]{F.~Kuehn}
\author[40,42]{D.~Kuempel}
\author[41]{J.K.~Kulbartz}
\author[37]{N.~Kunka}
\author[52]{G.~LaRosa}
\author[30]{C.~Lachaud}
\author[79]{D.~LaHurd}
\author[53]{L.~Latronico}
\author[94]{R.~Lauer}
\author[34]{P.~Lautridou}
\author[33]{S.~LeCoz}
\author[21]{M.S.A.B.~Le\~{a}o}
\author[33]{D.~Lebrun}
\author[83]{P.~Lebrun}
\author[21]{M.A.~Leigui de Oliveira}
\author[32]{A.~Letessier-Selvon}
\author[29]{I.~Lhenry-Yvon}
\author[38]{K.~Link}
\author[55]{R.~L\'{o}pez}
\author[75]{A.~Lopez Ag\"{u}era}
\author[33,31]{K.~Louedec}
\author[74]{J.~Lozano Bahilo}
\author[77]{L.~Lu}
\author[7]{A.~Lucero}
\author[38]{M.~Ludwig}
\author[22,29]{H.~Lyberis}
\author[52]{M.C.~Maccarone}
\author[32]{C.~Macolino}
\author[53]{S.~Maldera}
\author[26]{D.~Mandat}
\author[83]{P.~Mantsch}
\author[4]{A.G.~Mariazzi}
\author[9,53]{J.~Marin}
\author[34]{V.~Marin}
\author[32]{I.C.~Maris}
\author[57]{H.R.~Marquez Falcon}
\author[51]{G.~Marsella}
\author[46]{D.~Martello}
\author[34]{L.~Martin}
\author[56]{H.~Martinez}
\author[55]{O.~Mart\'{\i}nez Bravo}
\author[36]{H.J.~Mathes}
\author[85,91]{J.~Matthews}
\author[94]{J.A.J.~Matthews}
\author[48]{G.~Matthiae}
\author[36]{D.~Maurel}
\author[50]{D.~Maurizio}
\author[83]{P.O.~Mazur}
\author[58]{G.~Medina-Tanco}
\author[38]{M.~Melissas}
\author[7]{D.~Melo}
\author[50]{E.~Menichetti}
\author[37]{A.~Menshikov}
\author[76]{P.~Mertsch}
\author[40]{C.~Meurer}
\author[24]{S.~Mi'{c}anovi'{c}}
\author[6]{M.I.~Micheletti}
\author[72]{I.A.~Minaya}
\author[45]{L.~Miramonti}
\author[74]{L.~Molina-Bueno}
\author[1]{S.~Mollerach}
\author[92]{M.~Monasor}
\author[31]{D.~Monnier Ragaigne}
\author[33]{F.~Montanet}
\author[58]{B.~Morales}
\author[53]{C.~Morello}
\author[55]{E.~Moreno}
\author[4]{J.C.~Moreno}
\author[81]{M.~Mostaf\'{a}}
\author[21]{C.A.~Moura}
\author[17]{M.A.~Muller}
\author[40]{G.~M\"{u}ller}
\author[32]{M.~M\"{u}nchmeyer}
\author[50]{R.~Mussa}
% \author[53~‡]{G.~Navarra}
\author[74]{J.L.~Navarro}
\author[74]{S.~Navas}
\author[26]{P.~Necesal}
\author[58]{L.~Nellen}
\author[59,61]{A.~Nelles}
\author[35]{J.~Neuser}
\author[97]{P.T.~Nhung}
\author[42]{M.~Niechciol}
\author[35]{L.~Niemietz}
\author[35]{N.~Nierstenhoefer}
\author[86]{D.~Nitz}
\author[25]{D.~Nosek}
\author[26]{L.~No\v{z}ka}
\author[36]{J.~Oehlschl\"{a}ger}
\author[92]{A.~Olinto}
\author[72]{M.~Ortiz}
\author[73]{N.~Pacheco}
\author[17]{D.~Pakk Selmi-Dei}
\author[26]{M.~Palatka}
\author[2]{J.~Pallotta}
\author[38]{N.~Palmieri}
\author[75]{G.~Parente}
\author[30]{E.~Parizot}
\author[75]{A.~Parra}
\author[71]{S.~Pastor}
\author[88]{T.~Paul}
\author[26]{M.~Pech}
\author[63]{J.~P\c{e}kala}
\author[55,75]{R.~Pelayo}
\author[20]{I.M.~Pepe}
\author[51]{L.~Perrone}
\author[43]{R.~Pesce}
\author[93]{E.~Petermann}
\author[44]{S.~Petrera}
\author[43]{A.~Petrolini}
\author[81]{Y.~Petrov}
\author[95]{C.~Pfendner}
\author[3]{R.~Piegaia}
\author[36]{T.~Pierog}
\author[3]{P.~Pieroni}
\author[65]{M.~Pimenta}
\author[49]{V.~Pirronello}
\author[7]{M.~Platino}
\author[40]{M.~Plum}
\author[1]{V.H.~Ponce}
\author[42]{M.~Pontz}
\author[36]{A.~Porcelli}
\author[92]{P.~Privitera}
\author[26]{M.~Prouza}
\author[2]{E.J.~Quel}
\author[35]{S.~Querchfeld}
\author[35]{J.~Rautenberg}
\author[34]{O.~Ravel}
\author[7]{D.~Ravignani}
\author[34]{B.~Revenu}
\author[26]{J.~Ridky}
\author[75]{S.~Riggi}
\author[42]{M.~Risse}
\author[2]{P.~Ristori}
\author[45]{H.~Rivera}
\author[44]{V.~Rizi}
\author[87]{J.~Roberts}
\author[75]{W.~Rodriguesde Carvalho}
\author[75]{G.~Rodriguez}
\author[75]{I.~Rodriguez Cabo}
\author[9]{J.~Rodriguez Martino}
\author[9]{J.~Rodriguez Rojo}
\author[73]{M.D.~Rodr\'{\i}guez-Fr\'{\i}as}
\author[73]{G.~Ros}
\author[72]{J.~Rosado}
\author[27]{T.~Rossler}
\author[36]{M.~Roth}
\author[92]{B.~Rouill\'{e}-d'Orfeuil}
\author[1]{E.~Roulet}
\author[5]{A.C.~Rovero}
\author[37]{C.~R\"{u}hle}
\author[66]{A.~Saftoiu}
\author[29]{F.~Salamida}
\author[55]{H.~Salazar}
\author[81]{F.~Salesa Greus}
\author[48]{G.~Salina}
\author[7]{F.~S\'{a}nchez}
\author[65]{C.E.~Santo}
\author[65]{E.~Santos}
\author[22]{E.M.~Santos}
\author[80]{F.~Sarazin}
\author[35]{B.~Sarkar}
\author[76]{S.~Sarkar}
\author[9]{R.~Sato}
\author[40]{N.~Scharf}
\author[45]{V.~Scherini}
\author[36]{H.~Schieler}
\author[41,40]{P.~Schiffer}
\author[37]{A.~Schmidt}
\author[60]{O.~Scholten}
\author[59,61]{H.~Schoorlemmer}
\author[26]{J.~Schovancova}
\author[26]{P.~Schov\'{a}nek}
\author[36]{F.~Schr\"{o}der}
\author[40]{S.~Schulte}
\author[80]{D.~Schuster}
\author[4]{S.J.~Sciutto}
\author[49]{M.~Scuderi}
\author[52]{A.~Segreto}
\author[42]{M.~Settimo}
\author[85]{A.~Shadkam}
\author[14]{R.C.~Shellard}
\author[7]{I.~Sidelnik}
\author[41]{G.~Sigl}
\author[58]{H.H.~SilvaLopez}
\author[67]{O.~Sima}
\author[64]{A.~\'{S}mia\l kowski}
\author[36]{R.~\v{S}m\'{\i}da}
\author[93]{G.R.~Snow}
\author[90]{P.~Sommers}
\author[12]{J.~Sorokin}
\author[78,83]{H.~Spinka}
\author[9]{R.~Squartini}
\author[88]{Y.N.~Srivastava}
\author[70]{S.~Stanic}
\author[89]{J.~Stapleton}
\author[63]{J.~Stasielak}
\author[40]{M.~Stephan}
\author[33]{A.~Stutz}
\author[7]{F.~Suarez}
\author[29]{T.~Suomij\"{a}rvi}
\author[5]{A.D.~Supanitsky}
\author[24]{T.~\v{S}u\v{s}a}
\author[85]{M.S.~Sutherland}
\author[88]{J.~Swain}
\author[64]{Z.~Szadkowski}
\author[36]{M.~Szuba}
\author[7]{A.~Tapia}
\author[33]{M.~Tartare}
\author[35]{O.~Ta\c{s}c\u{a}u}
\author[42]{R.~Tcaciuc}
\author[97]{N.T.~Thao}
\author[81]{D.~Thomas}
\author[3]{J.~Tiffenberg}
\author[61,59]{C.~Timmermans}
\author[64]{W.~Tkaczyk}
\author[15]{C.J.~Todero Peixoto}
\author[66]{G.~Toma}
\author[26]{L.~Tomankova}
\author[65]{B.~Tom\'{e}}
\author[50]{A.~Tonachini}
\author[26]{P.~Travnicek}
\author[16]{D.B.~Tridapalli}
\author[30]{G.~Tristram}
\author[49]{E.~Trovato}
\author[75]{M.~Tueros}
\author[36]{R.~Ulrich}
\author[36]{M.~Unger}
\author[31]{M.~Urban}
\author[58]{J.F.~Vald\'{e}sGalicia}
\author[75]{I.~Vali\~{n}o}
\author[47]{L.~Valore}
\author[60]{A.M.~vandenBerg}
\author[55]{E.~Varela}
\author[58]{B.~VargasC\'{a}rdenas}
\author[72]{J.R.~V\'{a}zquez}
\author[75]{R.A.~V\'{a}zquez}
\author[70,69]{D.~Veberi\v{c}}
\author[48]{V.~Verzi}
\author[26]{J.~Vicha}
\author[8]{M.~Videla}
\author[57]{L.~Villase\~{n}or}
\author[4]{H.~Wahlberg}
\author[12]{P.~Wahrlich}
\author[7,11]{O.~Wainberg}
\author[40]{D.~Walz}
\author[77]{A.A.~Watson}
\author[37]{M.~Weber}
\author[40]{K.~Weidenhaupt}
\author[36]{A.~Weindl}
\author[36]{F.~Werner}
\author[95]{S.~Westerhoff}
\author[12]{B.J.~Whelan}
\author[88]{A.~Widom}
\author[64]{G.~Wieczorek}
\author[80]{L.~Wiencke}
\author[63]{B.~Wilczy\'{n}ska}
\author[63]{H.~Wilczy\'{n}ski}
\author[36]{M.~Will}
\author[92]{C.~Williams}
\author[40]{T.~Winchen}
\author[36]{M.~Wommer}
\author[7]{B.~Wundheiler}
% \author[92~a]{T.~Yamamoto}
\author[86]{T.~Yapici}
\author[42,84]{P.~Younk}
\author[85]{G.~Yuan}
\author[75]{A.~Yushkov}
\author[74]{B.~Zamorano Garcia}
\author[75]{E.~Zas}
\author[70,69]{D.~Zavrtanik}
\author[69,70]{M.~Zavrtanik}
% \author[87~h]{I.~Zaw}
\author[56]{A.~Zepeda}
\author[37]{Y.~Zhu}
\author[35,17]{M.~Zimbres Silva}
\author[42]{M.~Ziolkowski}

\address[1]{Centro At\'{o}mico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\address[2]{Centro de Investigaciones en L\'{a}seres y Aplicaciones, CITEDEF and CONICET, Argentina}
\address[3]{Departamento de F\'{\i}sica, FCEyN, Universidad de Buenos Aires y CONICET, Argentina}
\address[4]{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\address[5]{Instituto de Astronom\'{\i}a y F\'{\i}sica del Espacio (CONICET-UBA), Buenos Aires, Argentina}
\address[6]{Instituto de F\'{\i}sica de Rosario (IFIR) - CONICET/U.N.R. and Facultad de Ciencias Bioqu\'{\i}micas y Farmac\'{e}uticas U.N.R., Rosario, Argentina}
\address[7]{Instituto de Tecnolog\'{\i}as en Detecci\'{o}n y Astropart\'{\i}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\address[8]{National Technological University, Faculty Mendoza (CONICET/CNEA), Mendoza, Argentina}
\address[9]{Observatorio Pierre Auger, Malarg\"{u}e, Argentina}
\address[10]{Observatorio Pierre Auger and Comisi\'{o}n Nacional de Energ\'{\i}a At\'{o}mica, Malarg\"{u}e, Argentina}
\address[11]{Universidad Tecnol\'{o}gica Nacional - Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\address[12]{University of Adelaide, Adelaide, S.A., Australia}
\address[14]{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}
\address[15]{Universidade de S\~{a}o Paulo, Instituto de F\'{\i}sica, S\~{a}o Carlos, SP, Brazil}
\address[16]{Universidade de S\~{a}o Paulo, Instituto de F\'{\i}sica, S\~{a}o Paulo, SP, Brazil}
\address[17]{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\address[18]{Universidade Estadual de Feira de Santana, Brazil}
\address[19]{Universidade Estadual do Sudoeste da Bahia, Vitoria da Conquista, BA, Brazil}
\address[20]{Universidade Federal da Bahia, Salvador, BA, Brazil}
\address[21]{Universidade Federal do ABC, Santo Andr\'{e}, SP, Brazil}
\address[22]{Universidade Federal do Rio de Janeiro, Instituto de F\'{\i}sica, Rio de Janeiro, RJ, Brazil}
\address[23]{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}
\address[24]{Rudjer Bo\v{s}kovi'{c} Institute, 10000 Zagreb, Croatia}
\address[25]{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\address[26]{Institute of Physics of the Academy of Sciences of the Czech Republic, Prague, Czech Republic} 
\address[27]{Palacky University, RCPTM, Olomouc, Czech Republic}
\address[29]{Institut de Physique Nucl\'{e}aire d'Orsay (IPNO), Universit\'{e} Paris 11, CNRS-IN2P3, Orsay, France} 
\address[30]{Laboratoire AstroParticule et Cosmologie (APC), Universit\'{e} Paris 7, CNRS-IN2P3, Paris, France} 
\address[31]{Laboratoire de l'Acc\'{e}l\'{e}rateur Lin\'{e}aire (LAL), Universit\'{e} Paris 11, CNRS-IN2P3, Orsay, France}
\address[32]{Laboratoire de Physique Nucl\'{e}aire et de Hautes Energies (LPNHE), Universit\'{e}s Paris 6 et Paris 7, CNRS-IN2P3, Paris, France}
\address[33]{Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'{e} Joseph Fourier, INPG, CNRS-IN2P3, Grenoble, France}
\address[34]{SUBATECH, \'{E}cole des Mines de Nantes, CNRS-IN2P3, Universit\'{e} de Nantes, Nantes, France}
\address[35]{Bergische Universit\"{a}t Wuppertal, Wuppertal, Germany}
\address[36]{Karlsruhe Institute of Technology - Campus North - Institut f\"{u}r Kernphysik, Karlsruhe, Germany}
\address[37]{Karlsruhe Institute of Technology - Campus North - Institut f\"{u}r Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
\address[38]{Karlsruhe Institute of Technology - Campus South - Institut f\"{u}r Experimentelle Kernphysik (IEKP), Karlsruhe, Germany}
\address[39]{Max-Planck-Institut f\"{u}r Radioastronomie, Bonn, Germany}
\address[40]{RWTH Aachen University, III. Physikalisches Institut A, Aachen, Germany}
\address[41]{Universit\"{a}t Hamburg, Hamburg, Germany}
\address[42]{Universit\"{a}t Siegen, Siegen, Germany}
\address[43]{Dipartimento di Fisica dell'Universit\`{a} and INFN, Genova, Italy}
\address[44]{Universit\`{a} dell'Aquila and INFN, L'Aquila, Italy}
\address[45]{Universit\`{a} di Milano and Sezione INFN, Milan, Italy}
\address[46]{Dipartimento di Fisica dell'Universit\`{a} del Salento and Sezione INFN, Lecce, Italy}
\address[47]{Universit\`{a} di Napoli "Federico II" and Sezione INFN, Napoli, Italy}
\address[48]{Universit\`{a} di Roma II "Tor Vergata" and Sezione INFN,  Roma, Italy}
\address[49]{Universit\`{a} di Catania and Sezione INFN, Catania, Italy}
\address[50]{Universit\`{a} di Torino and Sezione INFN, Torino, Italy}
\address[51]{Dipartimento di Ingegneria dell'Innovazione dell'Universit\`{a} del Salento and Sezione INFN, Lecce, Italy}
\address[52]{Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo (INAF), Palermo, Italy}
\address[53]{Istituto di Fisica dello Spazio Interplanetario (INAF), Universit\`{a} di Torino and Sezione INFN, Torino, Italy}
\address[54]{INFN, Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}
\address[55]{Benem\'{e}rita Universidad Aut\'{o}noma de Puebla, Puebla, Mexico}
\address[56]{Centro de Investigaci\'{o}n y de Estudios Avanzados del IPN (CINVESTAV), M\'{e}xico, D.F., Mexico}
\address[57]{Universidad Michoacana de San Nicolas de Hidalgo, Morelia, Michoacan, Mexico}
\address[58]{Universidad Nacional Autonoma de Mexico, Mexico, D.F., Mexico}
\address[59]{IMAPP, Radboud University Nijmegen, Netherlands} 
\address[60]{Kernfysisch Versneller Instituut, University of Groningen, Groningen, Netherlands}
\address[61]{Nikhef, Science Park, Amsterdam, Netherlands}
\address[62]{ASTRON, Dwingeloo, Netherlands}
\address[63]{Institute of Nuclear Physics PAN, Krakow, Poland}
\address[64]{University of \L \'{o}d\'{z}, \L \'{o}d\'{z}, Poland}
\address[65]{LIP and Instituto Superior T\'{e}cnico, Technical University of Lisbon, Portugal}
\address[66]{'Horia Hulubei' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\address[67]{University of Bucharest, Physics Department, Romania}
\address[68]{University Politehnica of Bucharest, Romania}
\address[69]{J. Stefan Institute, Ljubljana, Slovenia}
\address[70]{Laboratory for Astroparticle Physics, University of Nova Gorica, Slovenia}
\address[71]{Instituto de F\'{\i}sica Corpuscular, CSIC-Universitat de Val\`{e}ncia, Valencia, Spain}
\address[72]{Universidad Complutense de Madrid, Madrid, Spain}
\address[73]{Universidad de Alcal\'{a}, Alcal\'{a} de Henares (Madrid), Spain}
\address[74]{Universidad de Granada \&  C.A.F.P.E., Granada, Spain}
\address[75]{Universidad de Santiago de Compostela, Spain}
\address[76]{Rudolf Peierls Centre for Theoretical Physics, University of Oxford, Oxford, United Kingdom}
\address[77]{School of Physics and Astronomy, University of Leeds, United Kingdom}
\address[78]{Argonne National Laboratory, Argonne, IL, USA}
\address[79]{Case Western Reserve University, Cleveland, OH, USA}
\address[80]{Colorado School of Mines, Golden, CO, USA}
\address[81]{Colorado State University, Fort Collins, CO, USA} 
\address[82]{Colorado State University, Pueblo, CO, USA}
\address[83]{Fermilab, Batavia, IL, USA}
\address[84]{Los Alamos National Laboratory, Los Alamos, NM, USA}
\address[85]{Louisiana State University, Baton Rouge, LA, USA}
\address[86]{Michigan Technological University, Houghton, MI, USA}
\address[87]{New York University, New York, NY, USA}
\address[88]{Northeastern University, Boston, MA, USA}
\address[89]{Ohio State University, Columbus, OH, USA}
\address[90]{Pennsylvania State University, University Park, PA, USA}
\address[91]{Southern University, Baton Rouge, LA, USA}
\address[92]{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\address[93]{University of Nebraska, Lincoln, NE, USA}
\address[94]{University of New Mexico, Albuquerque, NM, USA}
\address[95]{University of Wisconsin, Madison, WI, USA}
\address[96]{University of Wisconsin, Milwaukee, WI, USA}
\address[97]{Institute for Nuclear Science and Technology (INST), Hanoi, Vietnam}

% (‡) Deceased \\
% (a) at Konan University, Kobe, Japan \\
% (f) now at University of Maryland \\
% (h) now at NYU Abu Dhabi \\
% (i) now at Universit\'{e} de Lausanne \\
% last updated:	2/3/2012 


==> author_list_latex2.tex <==
% This is a fragment that can be inserted into a LaTeX
\par\noindent
P.~Abreu$^{63}$, 
M.~Aglietta$^{51}$, 
M.~Ahlers$^{94}$, 
E.J.~Ahn$^{81}$, 
I.F.M.~Albuquerque$^{15}$, 
D.~Allard$^{29}$, 
I.~Allekotte$^{1}$, 
J.~Allen$^{85}$, 
P.~Allison$^{87}$, 
A.~Almela$^{11,\: 7}$, 
J.~Alvarez Castillo$^{56}$, 
J.~Alvarez-Mu\~{n}iz$^{73}$, 
R.~Alves Batista$^{16}$, 
M.~Ambrosio$^{45}$, 
A.~Aminaei$^{57}$, 
L.~Anchordoqui$^{95}$, 
S.~Andringa$^{63}$, 
T.~Anti\v{c}i'{c}$^{23}$, 
C.~Aramo$^{45}$, 
E.~Arganda$^{4,\: 70}$, 
F.~Arqueros$^{70}$, 
H.~Asorey$^{1}$, 
P.~Assis$^{63}$, 
J.~Aublin$^{31}$, 
M.~Ave$^{37}$, 
M.~Avenier$^{32}$, 
G.~Avila$^{10}$, 
A.M.~Badescu$^{66}$, 
M.~Balzer$^{36}$, 
K.B.~Barber$^{12}$, 
A.F.~Barbosa$^{13~\ddag}$, 
R.~Bardenet$^{30}$, 
S.L.C.~Barroso$^{18}$, 
B.~Baughman$^{87~f}$, 
J.~B\"{a}uml$^{35}$, 
C.~Baus$^{37}$, 
J.J.~Beatty$^{87}$, 
K.H.~Becker$^{34}$, 
A.~Bell\'{e}toile$^{33}$, 
J.A.~Bellido$^{12}$, 
S.~BenZvi$^{94}$, 
C.~Berat$^{32}$, 
X.~Bertou$^{1}$, 
P.L.~Biermann$^{38}$, 
P.~Billoir$^{31}$, 
F.~Blanco$^{70}$, 
M.~Blanco$^{31,\: 71}$, 
C.~Bleve$^{34}$, 
H.~Bl\"{u}mer$^{37,\: 35}$, 
M.~Boh\'{a}\v{c}ov\'{a}$^{25}$, 
D.~Boncioli$^{46}$, 
C.~Bonifazi$^{21,\: 31}$, 
R.~Bonino$^{51}$, 
N.~Borodai$^{61}$, 
J.~Brack$^{79}$, 
I.~Brancus$^{64}$, 
P.~Brogueira$^{63}$, 
W.C.~Brown$^{80}$, 
R.~Bruijn$^{75~i}$, 
P.~Buchholz$^{41}$, 
A.~Bueno$^{72}$, 
L.~Buroker$^{95}$, 
R.E.~Burton$^{77}$, 
K.S.~Caballero-Mora$^{88}$, 
B.~Caccianiga$^{44}$, 
L.~Caramete$^{38}$, 
R.~Caruso$^{47}$, 
A.~Castellina$^{51}$, 
O.~Catalano$^{50}$, 
G.~Cataldi$^{49}$, 
L.~Cazon$^{63}$, 
R.~Cester$^{48}$, 
J.~Chauvin$^{32}$, 
S.H.~Cheng$^{88}$, 
A.~Chiavassa$^{51}$, 
J.A.~Chinellato$^{16}$, 
J.~Chirinos Diaz$^{84}$, 
J.~Chudoba$^{25}$, 
M.~Cilmo$^{45}$, 
R.W.~Clay$^{12}$, 
G.~Cocciolo$^{49}$, 
L.~Collica$^{44}$, 
M.R.~Coluccia$^{49}$, 
R.~Concei\c{c}\~{a}o$^{63}$, 
F.~Contreras$^{9}$, 
H.~Cook$^{75}$, 
M.J.~Cooper$^{12}$, 
J.~Coppens$^{57,\: 59}$, 
A.~Cordier$^{30}$, 
S.~Coutu$^{88}$, 
C.E.~Covault$^{77}$, 
A.~Creusot$^{29}$, 
A.~Criss$^{88}$, 
J.~Cronin$^{90}$, 
A.~Curutiu$^{38}$, 
S.~Dagoret-Campagne$^{30}$, 
R.~Dallier$^{33}$, 
B.~Daniel$^{16}$, 
S.~Dasso$^{5,\: 3}$, 
K.~Daumiller$^{35}$, 
B.R.~Dawson$^{12}$, 
R.M.~de Almeida$^{22}$, 
M.~De Domenico$^{47}$, 
C.~De Donato$^{56}$, 
S.J.~de Jong$^{57,\: 59}$, 
G.~De La Vega$^{8}$, 
W.J.M.~de Mello Junior$^{16}$, 
J.R.T.~de Mello Neto$^{21}$, 
I.~De Mitri$^{49}$, 
V.~de Souza$^{14}$, 
K.D.~de Vries$^{58}$, 
L.~del Peral$^{71}$, 
M.~del R\'{\i}o$^{46,\: 9}$, 
O.~Deligny$^{28}$, 
H.~Dembinski$^{37}$, 
N.~Dhital$^{84}$, 
C.~Di Giulio$^{46,\: 43}$, 
M.L.~D\'{\i}az Castro$^{13}$, 
P.N.~Diep$^{96}$, 
F.~Diogo$^{63}$, 
C.~Dobrigkeit $^{16}$, 
W.~Docters$^{58}$, 
J.C.~D'Olivo$^{56}$, 
P.N.~Dong$^{96,\: 28}$, 
A.~Dorofeev$^{79}$, 
J.C.~dos Anjos$^{13}$, 
M.T.~Dova$^{4}$, 
D.~D'Urso$^{45}$, 
I.~Dutan$^{38}$, 
J.~Ebr$^{25}$, 
R.~Engel$^{35}$, 
M.~Erdmann$^{39}$, 
C.O.~Escobar$^{81,\: 16}$, 
J.~Espadanal$^{63}$, 
A.~Etchegoyen$^{7,\: 11}$, 
P.~Facal San Luis$^{90}$, 
H.~Falcke$^{57,\: 60,\: 59}$, 
G.~Farrar$^{85}$, 
A.C.~Fauth$^{16}$, 
N.~Fazzini$^{81}$, 
A.P.~Ferguson$^{77}$, 
B.~Fick$^{84}$, 
J.M.~Figueira$^{7}$, 
A.~Filevich$^{7}$, 
A.~Filip\v{c}i\v{c}$^{67,\: 68}$, 
S.~Fliescher$^{39}$, 
C.E.~Fracchiolla$^{79}$, 
E.D.~Fraenkel$^{58}$, 
O.~Fratu$^{66}$, 
U.~Fr\"{o}hlich$^{41}$, 
B.~Fuchs$^{37}$, 
R.~Gaior$^{31}$, 
R.F.~Gamarra$^{7}$, 
S.~Gambetta$^{42}$, 
B.~Garc\'{\i}a$^{8}$, 
S.T.~Garcia Roca$^{73}$, 
D.~Garcia-Gamez$^{30}$, 
D.~Garcia-Pinto$^{70}$, 
A.~Gascon Bravo$^{72}$, 
H.~Gemmeke$^{36}$, 
P.L.~Ghia$^{31}$, 
M.~Giller$^{62}$, 
J.~Gitto$^{8}$, 
H.~Glass$^{81}$, 
M.S.~Gold$^{93}$, 
G.~Golup$^{1}$, 
F.~Gomez Albarracin$^{4}$, 
M.~G\'{o}mez Berisso$^{1}$, 
P.F.~G\'{o}mez Vitale$^{10}$, 
P.~Gon\c{c}alves$^{63}$, 
J.G.~Gonzalez$^{35}$, 
B.~Gookin$^{79}$, 
A.~Gorgi$^{51}$, 
P.~Gouffon$^{15}$, 
E.~Grashorn$^{87}$, 
S.~Grebe$^{57,\: 59}$, 
N.~Griffith$^{87}$, 
M.~Grigat$^{39}$, 
A.F.~Grillo$^{52}$, 
Y.~Guardincerri$^{3}$, 
F.~Guarino$^{45}$, 
G.P.~Guedes$^{17}$, 
P.~Hansen$^{4}$, 
D.~Harari$^{1}$, 
T.A.~Harrison$^{12}$, 
J.L.~Harton$^{79}$, 
A.~Haungs$^{35}$, 
T.~Hebbeker$^{39}$, 
D.~Heck$^{35}$, 
A.E.~Herve$^{12}$, 
C.~Hojvat$^{81}$, 
N.~Hollon$^{90}$, 
V.C.~Holmes$^{12}$, 
P.~Homola$^{61}$, 
J.R.~H\"{o}randel$^{57,\: 59}$, 
P.~Horvath$^{26}$, 
M.~Hrabovsk\'{y}$^{26,\: 25}$, 
D.~Huber$^{37}$, 
T.~Huege$^{35}$, 
A.~Insolia$^{47}$, 
F.~Ionita$^{90}$, 
A.~Italiano$^{47}$, 
S.~Jansen$^{57,\: 59}$, 
C.~Jarne$^{4}$, 
S.~Jiraskova$^{57}$, 
M.~Josebachuili$^{7}$, 
K.~Kadija$^{23}$, 
K.H.~Kampert$^{34}$, 
P.~Karhan$^{24}$, 
P.~Kasper$^{81}$, 
I.~Katkov$^{37}$, 
B.~K\'{e}gl$^{30}$, 
B.~Keilhauer$^{35}$, 
A.~Keivani$^{83}$, 
J.L.~Kelley$^{57}$, 
E.~Kemp$^{16}$, 
R.M.~Kieckhafer$^{84}$, 
H.O.~Klages$^{35}$, 
M.~Kleifges$^{36}$, 
J.~Kleinfeller$^{9,\: 35}$, 
J.~Knapp$^{75}$, 
D.-H.~Koang$^{32}$, 
K.~Kotera$^{90}$, 
N.~Krohm$^{34}$, 
O.~Kr\"{o}mer$^{36}$, 
D.~Kruppke-Hansen$^{34}$, 
D.~Kuempel$^{39,\: 41}$, 
J.K.~Kulbartz$^{40}$, 
N.~Kunka$^{36}$, 
G.~La Rosa$^{50}$, 
C.~Lachaud$^{29}$, 
D.~LaHurd$^{77}$, 
L.~Latronico$^{51}$, 
R.~Lauer$^{93}$, 
P.~Lautridou$^{33}$, 
S.~Le Coz$^{32}$, 
M.S.A.B.~Le\~{a}o$^{20}$, 
D.~Lebrun$^{32}$, 
P.~Lebrun$^{81}$, 
M.A.~Leigui de Oliveira$^{20}$, 
A.~Letessier-Selvon$^{31}$, 
I.~Lhenry-Yvon$^{28}$, 
K.~Link$^{37}$, 
R.~L\'{o}pez$^{53}$, 
A.~Lopez Ag\"{u}era$^{73}$, 
K.~Louedec$^{32,\: 30}$, 
J.~Lozano Bahilo$^{72}$, 
L.~Lu$^{75}$, 
A.~Lucero$^{7}$, 
M.~Ludwig$^{37}$, 
H.~Lyberis$^{21,\: 28}$, 
M.C.~Maccarone$^{50}$, 
C.~Macolino$^{31}$, 
S.~Maldera$^{51}$, 
J.~Maller$^{33}$, 
D.~Mandat$^{25}$, 
P.~Mantsch$^{81}$, 
A.G.~Mariazzi$^{4}$, 
J.~Marin$^{9,\: 51}$, 
V.~Marin$^{33}$, 
I.C.~Maris$^{31}$, 
H.R.~Marquez Falcon$^{55}$, 
G.~Marsella$^{49}$, 
D.~Martello$^{49}$, 
L.~Martin$^{33}$, 
H.~Martinez$^{54}$, 
O.~Mart\'{\i}nez Bravo$^{53}$, 
D.~Martraire$^{28}$, 
J.J.~Mas\'{\i}as Meza$^{3}$, 
H.J.~Mathes$^{35}$, 
J.~Matthews$^{83,\: 89}$, 
J.A.J.~Matthews$^{93}$, 
G.~Matthiae$^{46}$, 
D.~Maurel$^{35}$, 
D.~Maurizio$^{13,\: 48}$, 
P.O.~Mazur$^{81}$, 
G.~Medina-Tanco$^{56}$, 
M.~Melissas$^{37}$, 
D.~Melo$^{7}$, 
E.~Menichetti$^{48}$, 
A.~Menshikov$^{36}$, 
P.~Mertsch$^{74}$, 
C.~Meurer$^{39}$, 
R.~Meyhandan$^{91}$, 
S.~Mi'{c}anovi'{c}$^{23}$, 
M.I.~Micheletti$^{6}$, 
I.A.~Minaya$^{70}$, 
L.~Miramonti$^{44}$, 
L.~Molina-Bueno$^{72}$, 
S.~Mollerach$^{1}$, 
M.~Monasor$^{90}$, 
D.~Monnier Ragaigne$^{30}$, 
F.~Montanet$^{32}$, 
B.~Morales$^{56}$, 
C.~Morello$^{51}$, 
E.~Moreno$^{53}$, 
J.C.~Moreno$^{4}$, 
M.~Mostaf\'{a}$^{79}$, 
C.A.~Moura$^{20}$, 
M.A.~Muller$^{16}$, 
G.~M\"{u}ller$^{39}$, 
M.~M\"{u}nchmeyer$^{31}$, 
R.~Mussa$^{48}$, 
G.~Navarra$^{51~\ddag}$, 
J.L.~Navarro$^{72}$, 
S.~Navas$^{72}$, 
P.~Necesal$^{25}$, 
L.~Nellen$^{56}$, 
A.~Nelles$^{57,\: 59}$, 
J.~Neuser$^{34}$, 
P.T.~Nhung$^{96}$, 
M.~Niechciol$^{41}$, 
L.~Niemietz$^{34}$, 
N.~Nierstenhoefer$^{34}$, 
D.~Nitz$^{84}$, 
D.~Nosek$^{24}$, 
L.~No\v{z}ka$^{25}$, 
J.~Oehlschl\"{a}ger$^{35}$, 
A.~Olinto$^{90}$, 
M.~Ortiz$^{70}$, 
N.~Pacheco$^{71}$, 
D.~Pakk Selmi-Dei$^{16}$, 
M.~Palatka$^{25}$, 
J.~Pallotta$^{2}$, 
N.~Palmieri$^{37}$, 
G.~Parente$^{73}$, 
E.~Parizot$^{29}$, 
A.~Parra$^{73}$, 
S.~Pastor$^{69}$, 
T.~Paul$^{86}$, 
M.~Pech$^{25}$, 
J.~P\c{e}kala$^{61}$, 
R.~Pelayo$^{53,\: 73}$, 
I.M.~Pepe$^{19}$, 
L.~Perrone$^{49}$, 
R.~Pesce$^{42}$, 
E.~Petermann$^{92}$, 
S.~Petrera$^{43}$, 
A.~Petrolini$^{42}$, 
Y.~Petrov$^{79}$, 
C.~Pfendner$^{94}$, 
R.~Piegaia$^{3}$, 
T.~Pierog$^{35}$, 
P.~Pieroni$^{3}$, 
M.~Pimenta$^{63}$, 
V.~Pirronello$^{47}$, 
M.~Platino$^{7}$, 
M.~Plum$^{39}$, 
V.H.~Ponce$^{1}$, 
M.~Pontz$^{41}$, 
A.~Porcelli$^{35}$, 
P.~Privitera$^{90}$, 
M.~Prouza$^{25}$, 
E.J.~Quel$^{2}$, 
S.~Querchfeld$^{34}$, 
J.~Rautenberg$^{34}$, 
O.~Ravel$^{33}$, 
D.~Ravignani$^{7}$, 
B.~Revenu$^{33}$, 
J.~Ridky$^{25}$, 
S.~Riggi$^{73}$, 
M.~Risse$^{41}$, 
P.~Ristori$^{2}$, 
H.~Rivera$^{44}$, 
V.~Rizi$^{43}$, 
J.~Roberts$^{85}$, 
W.~Rodrigues de Carvalho$^{73}$, 
G.~Rodriguez$^{73}$, 
I.~Rodriguez Cabo$^{73}$, 
J.~Rodriguez Martino$^{9}$, 
J.~Rodriguez Rojo$^{9}$, 
M.D.~Rodr\'{\i}guez-Fr\'{\i}as$^{71}$, 
G.~Ros$^{71}$, 
J.~Rosado$^{70}$, 
T.~Rossler$^{26}$, 
M.~Roth$^{35}$, 
B.~Rouill\'{e}-d'Orfeuil$^{90}$, 
E.~Roulet$^{1}$, 
A.C.~Rovero$^{5}$, 
C.~R\"{u}hle$^{36}$, 
A.~Saftoiu$^{64}$, 
F.~Salamida$^{28}$, 
H.~Salazar$^{53}$, 
F.~Salesa Greus$^{79}$, 
G.~Salina$^{46}$, 
F.~S\'{a}nchez$^{7}$, 
C.E.~Santo$^{63}$, 
E.~Santos$^{63}$, 
E.M.~Santos$^{21}$, 
F.~Sarazin$^{78}$, 
B.~Sarkar$^{34}$, 
S.~Sarkar$^{74}$, 
R.~Sato$^{9}$, 
N.~Scharf$^{39}$, 
V.~Scherini$^{44}$, 
H.~Schieler$^{35}$, 
P.~Schiffer$^{40,\: 39}$, 
A.~Schmidt$^{36}$, 
O.~Scholten$^{58}$, 
H.~Schoorlemmer$^{57,\: 59}$, 
J.~Schovancova$^{25}$, 
P.~Schov\'{a}nek$^{25}$, 
F.~Schr\"{o}der$^{35}$, 
S.~Schulte$^{39}$, 
D.~Schuster$^{78}$, 
S.J.~Sciutto$^{4}$, 
M.~Scuderi$^{47}$, 
A.~Segreto$^{50}$, 
M.~Settimo$^{41}$, 
A.~Shadkam$^{83}$, 
R.C.~Shellard$^{13}$, 
I.~Sidelnik$^{7}$, 
G.~Sigl$^{40}$, 
H.H.~Silva Lopez$^{56}$, 
O.~Sima$^{65}$, 
A.~'{S}mia\l kowski$^{62}$, 
R.~\v{S}m\'{\i}da$^{35}$, 
G.R.~Snow$^{92}$, 
P.~Sommers$^{88}$, 
J.~Sorokin$^{12}$, 
H.~Spinka$^{76,\: 81}$, 
R.~Squartini$^{9}$, 
Y.N.~Srivastava$^{86}$, 
S.~Stanic$^{68}$, 
J.~Stapleton$^{87}$, 
J.~Stasielak$^{61}$, 
M.~Stephan$^{39}$, 
A.~Stutz$^{32}$, 
F.~Suarez$^{7}$, 
T.~Suomij\"{a}rvi$^{28}$, 
A.D.~Supanitsky$^{5}$, 
T.~\v{S}u\v{s}a$^{23}$, 
M.S.~Sutherland$^{83}$, 
J.~Swain$^{86}$, 
Z.~Szadkowski$^{62}$, 
M.~Szuba$^{35}$, 
A.~Tapia$^{7}$, 
M.~Tartare$^{32}$, 
O.~Ta\c{s}c\u{a}u$^{34}$, 
R.~Tcaciuc$^{41}$, 
N.T.~Thao$^{96}$, 
D.~Thomas$^{79}$, 
J.~Tiffenberg$^{3}$, 
C.~Timmermans$^{59,\: 57}$, 
W.~Tkaczyk$^{62~\ddag}$, 
C.J.~Todero Peixoto$^{14}$, 
G.~Toma$^{64}$, 
L.~Tomankova$^{25}$, 
B.~Tom\'{e}$^{63}$, 
A.~Tonachini$^{48}$, 
P.~Travnicek$^{25}$, 
D.B.~Tridapalli$^{15}$, 
G.~Tristram$^{29}$, 
E.~Trovato$^{47}$, 
M.~Tueros$^{73}$, 
R.~Ulrich$^{35}$, 
M.~Unger$^{35}$, 
M.~Urban$^{30}$, 
J.F.~Vald\'{e}s Galicia$^{56}$, 
I.~Vali\~{n}o$^{73}$, 
L.~Valore$^{45}$, 
G.~van Aar$^{57}$, 
A.M.~van den Berg$^{58}$, 
A.~van Vliet$^{40}$, 
E.~Varela$^{53}$, 
B.~Vargas C\'{a}rdenas$^{56}$, 
J.R.~V\'{a}zquez$^{70}$, 
R.A.~V\'{a}zquez$^{73}$, 
D.~Veberi\v{c}$^{68,\: 67}$, 
V.~Verzi$^{46}$, 
J.~Vicha$^{25}$, 
M.~Videla$^{8}$, 
L.~Villase\~{n}or$^{55}$, 
H.~Wahlberg$^{4}$, 
P.~Wahrlich$^{12}$, 
O.~Wainberg$^{7,\: 11}$, 
D.~Walz$^{39}$, 
A.A.~Watson$^{75}$, 
M.~Weber$^{36}$, 
K.~Weidenhaupt$^{39}$, 
A.~Weindl$^{35}$, 
F.~Werner$^{35}$, 
S.~Westerhoff$^{94}$, 
B.J.~Whelan$^{88,\: 12}$, 
A.~Widom$^{86}$, 
G.~Wieczorek$^{62}$, 
L.~Wiencke$^{78}$, 
B.~Wilczy\'{n}ska$^{61}$, 
H.~Wilczy\'{n}ski$^{61}$, 
M.~Will$^{35}$, 
C.~Williams$^{90}$, 
T.~Winchen$^{39}$, 
M.~Wommer$^{35}$, 
B.~Wundheiler$^{7}$, 
T.~Yamamoto$^{90~a}$, 
T.~Yapici$^{84}$, 
P.~Younk$^{41,\: 82}$, 
G.~Yuan$^{83}$, 
A.~Yushkov$^{73}$, 
B.~Zamorano Garcia$^{72}$, 
E.~Zas$^{73}$, 
D.~Zavrtanik$^{68,\: 67}$, 
M.~Zavrtanik$^{67,\: 68}$, 
I.~Zaw$^{85~h}$, 
A.~Zepeda$^{54~b}$, 
J.~Zhou$^{90}$, 
Y.~Zhu$^{36}$, 
M.~Zimbres Silva$^{34,\: 16}$, 
M.~Ziolkowski$^{41}$
% \newline% 
% \vskip 0.05cm
\begin{center}
(The Pierre Auger Collaboration)      
% \centering
\vskip 0.75cm
and
D.~Charrier$^{33}$,
L.~Denis$^{j}$,
G.~Hilgers$^{39}$,
O.~Kr\"omer$^{36}$,
L.~Mohrmann$^{39}$,
B.~Philipps$^{39}$,
O.~Seeger$^{39}$
% \newpage% 
\end{center}

\vskip 0.5cm
\begin{flushleft}
\begin{itshape}
\begin{small}
\par\noindent
$^{1}$ Centro At\'{o}mico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San 
Carlos de Bariloche, 
Argentina \\
$^{2}$ Centro de Investigaciones en L\'{a}seres y Aplicaciones, CITEDEF and CONICET, 
Argentina \\
$^{3}$ Departamento de F\'{\i}sica, FCEyN, Universidad de Buenos Aires y CONICET, 
Argentina \\
$^{4}$ IFLP, Universidad Nacional de La Plata and CONICET, La Plata, 
Argentina \\
$^{5}$ Instituto de Astronom\'{\i}a y F\'{\i}sica del Espacio (CONICET-UBA), Buenos Aires, 
Argentina \\
$^{6}$ Instituto de F\'{\i}sica de Rosario (IFIR) - CONICET/U.N.R. and Facultad de Ciencias 
Bioqu\'{\i}micas y Farmac\'{e}uticas U.N.R., Rosario, 
Argentina \\
$^{7}$ Instituto de Tecnolog\'{\i}as en Detecci\'{o}n y Astropart\'{\i}culas (CNEA, CONICET, UNSAM), 
Buenos Aires, 
Argentina \\
$^{8}$ National Technological University, Faculty Mendoza (CONICET/CNEA), Mendoza, 
Argentina \\
$^{9}$ Observatorio Pierre Auger, Malarg\"{u}e, 
Argentina \\
$^{10}$ Observatorio Pierre Auger and Comisi\'{o}n Nacional de Energ\'{\i}a At\'{o}mica, Malarg\"{u}e, 
Argentina \\
$^{11}$ Universidad Tecnol\'{o}gica Nacional - Facultad Regional Buenos Aires, Buenos Aires,
Argentina \\
$^{12}$ University of Adelaide, Adelaide, S.A., 
Australia \\
$^{13}$ Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, 
Brazil \\
$^{14}$ Universidade de S\~{a}o Paulo, Instituto de F\'{\i}sica, S\~{a}o Carlos, SP, 
Brazil \\
$^{15}$ Universidade de S\~{a}o Paulo, Instituto de F\'{\i}sica, S\~{a}o Paulo, SP, 
Brazil \\
$^{16}$ Universidade Estadual de Campinas, IFGW, Campinas, SP, 
Brazil \\
$^{17}$ Universidade Estadual de Feira de Santana, 
Brazil \\
$^{18}$ Universidade Estadual do Sudoeste da Bahia, Vitoria da Conquista, BA, 
Brazil \\
$^{19}$ Universidade Federal da Bahia, Salvador, BA, 
Brazil \\
$^{20}$ Universidade Federal do ABC, Santo Andr\'{e}, SP, 
Brazil \\
$^{21}$ Universidade Federal do Rio de Janeiro, Instituto de F\'{\i}sica, Rio de Janeiro, RJ, 
Brazil \\
$^{22}$ Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, 
Brazil \\
$^{23}$ Rudjer Bo\v{s}kovi'{c} Institute, 10000 Zagreb, 
Croatia \\
$^{24}$ Charles University, Faculty of Mathematics and Physics, Institute of Particle and 
Nuclear Physics, Prague, 
Czech Republic \\
$^{25}$ Institute of Physics of the Academy of Sciences of the Czech Republic, Prague, 
Czech Republic \\
$^{26}$ Palacky University, RCPTM, Olomouc, 
Czech Republic \\
$^{28}$ Institut de Physique Nucl\'{e}aire d'Orsay (IPNO), Universit\'{e} Paris 11, CNRS-IN2P3, 
Orsay, 
France \\
$^{29}$ Laboratoire AstroParticule et Cosmologie (APC), Universit\'{e} Paris 7, CNRS-IN2P3, 
Paris, 
France \\
$^{30}$ Laboratoire de l'Acc\'{e}l\'{e}rateur Lin\'{e}aire (LAL), Universit\'{e} Paris 11, CNRS-IN2P3, 
France \\
$^{31}$ Laboratoire de Physique Nucl\'{e}aire et de Hautes Energies (LPNHE), Universit\'{e}s 
Paris 6 et Paris 7, CNRS-IN2P3, Paris, 
France \\
$^{32}$ Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'{e} Joseph
 Fourier, INPG, CNRS-IN2P3, Grenoble, 
France \\
$^{33}$ SUBATECH, \'{E}cole des Mines de Nantes, CNRS-IN2P3, Universit\'{e} de Nantes, 
France \\
$^{34}$ Bergische Universit\"{a}t Wuppertal, Wuppertal, 
Germany \\
$^{35}$ Karlsruhe Institute of Technology - Campus North - Institut f\"{u}r Kernphysik, Karlsruhe, 
Germany \\
$^{36}$ Karlsruhe Institute of Technology - Campus North - Institut f\"{u}r 
Prozessdatenverarbeitung und Elektronik, Karlsruhe, 
Germany \\
$^{37}$ Karlsruhe Institute of Technology - Campus South - Institut f\"{u}r Experimentelle 
Kernphysik (IEKP), Karlsruhe, 
Germany \\
$^{38}$ Max-Planck-Institut f\"{u}r Radioastronomie, Bonn, 
Germany \\
$^{39}$ RWTH Aachen University, III. Physikalisches Institut A, Aachen, 
Germany \\
$^{40}$ Universit\"{a}t Hamburg, Hamburg, 
Germany \\
$^{41}$ Universit\"{a}t Siegen, Siegen, 
Germany \\
$^{42}$ Dipartimento di Fisica dell'Universit\`{a} and INFN, Genova, 
Italy \\
$^{43}$ Universit\`{a} dell'Aquila and INFN, L'Aquila, 
Italy \\
$^{44}$ Universit\`{a} di Milano and Sezione INFN, Milan, 
Italy \\
$^{45}$ Universit\`{a} di Napoli "Federico II" and Sezione INFN, Napoli, 
Italy \\
$^{46}$ Universit\`{a} di Roma II "Tor Vergata" and Sezione INFN,  Roma, 
Italy \\
$^{47}$ Universit\`{a} di Catania and Sezione INFN, Catania, 
Italy \\
$^{48}$ Universit\`{a} di Torino and Sezione INFN, Torino, 
Italy \\
$^{49}$ Dipartimento di Matematica e Fisica "E. De Giorgi" dell'Universit\`{a} del Salento and 
Sezione INFN, Lecce, 
Italy \\
$^{50}$ Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo (INAF), Palermo, 
Italy \\
$^{51}$ Istituto di Fisica dello Spazio Interplanetario (INAF), Universit\`{a} di Torino and 
Sezione INFN, Torino, 
Italy \\
$^{52}$ INFN, Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), 
Italy \\
$^{53}$ Benem\'{e}rita Universidad Aut\'{o}noma de Puebla, Puebla, 
Mexico \\
$^{54}$ Centro de Investigaci\'{o}n y de Estudios Avanzados del IPN (CINVESTAV), M\'{e}xico, 
Mexico \\
$^{55}$ Universidad Michoacana de San Nicolas de Hidalgo, Morelia, Michoacan, 
Mexico \\
$^{56}$ Universidad Nacional Autonoma de Mexico, Mexico, D.F., 
Mexico \\
$^{57}$ IMAPP, Radboud University Nijmegen, 
Netherlands \\
$^{58}$ Kernfysisch Versneller Instituut, University of Groningen, Groningen, 
Netherlands \\
$^{59}$ Nikhef, Science Park, Amsterdam, 
Netherlands \\
$^{60}$ ASTRON, Dwingeloo, 
Netherlands \\
$^{61}$ Institute of Nuclear Physics PAN, Krakow, 
Poland \\
$^{62}$ University of \L \'{o}d\'{z}, \L \'{o}d\'{z}, 
Poland \\
$^{63}$ LIP and Instituto Superior T\'{e}cnico, Technical University of Lisbon, 
Portugal \\
$^{64}$ 'Horia Hulubei' National Institute for Physics and Nuclear Engineering, Bucharest-
Magurele, 
Romania \\
$^{65}$ University of Bucharest, Physics Department, 
Romania \\
$^{66}$ University Politehnica of Bucharest, 
Romania \\
$^{67}$ J. Stefan Institute, Ljubljana, 
Slovenia \\
$^{68}$ Laboratory for Astroparticle Physics, University of Nova Gorica, 
Slovenia \\
$^{69}$ Instituto de F\'{\i}sica Corpuscular, CSIC-Universitat de Val\`{e}ncia, Valencia, 
Spain \\
$^{70}$ Universidad Complutense de Madrid, Madrid, 
Spain \\
$^{71}$ Universidad de Alcal\'{a}, Alcal\'{a} de Henares (Madrid), 
Spain \\
$^{72}$ Universidad de Granada \&  C.A.F.P.E., Granada, 
Spain \\
$^{73}$ Universidad de Santiago de Compostela, 
Spain \\
$^{74}$ Rudolf Peierls Centre for Theoretical Physics, University of Oxford, Oxford, 
United Kingdom \\
$^{75}$ School of Physics and Astronomy, University of Leeds, 
United Kingdom \\
$^{76}$ Argonne National Laboratory, Argonne, IL, 
USA \\
$^{77}$ Case Western Reserve University, Cleveland, OH, 
USA \\
$^{78}$ Colorado School of Mines, Golden, CO, 
USA \\
$^{79}$ Colorado State University, Fort Collins, CO, 
USA \\
$^{80}$ Colorado State University, Pueblo, CO, 
USA \\
$^{81}$ Fermilab, Batavia, IL, 
USA \\
$^{82}$ Los Alamos National Laboratory, Los Alamos, NM, 
USA \\
$^{83}$ Louisiana State University, Baton Rouge, LA, 
USA \\
$^{84}$ Michigan Technological University, Houghton, MI, 
USA \\
$^{85}$ New York University, New York, NY, 
USA \\
$^{86}$ Northeastern University, Boston, MA, 
USA \\
$^{87}$ Ohio State University, Columbus, OH, 
USA \\
$^{88}$ Pennsylvania State University, University Park, PA, 
USA \\
$^{89}$ Southern University, Baton Rouge, LA, 
USA \\
$^{90}$ University of Chicago, Enrico Fermi Institute, Chicago, IL, 
USA \\
$^{91}$ University of Hawaii, Honolulu, HI, 
USA \\
$^{92}$ University of Nebraska, Lincoln, NE, 
USA \\
$^{93}$ University of New Mexico, Albuquerque, NM, 
USA \\
$^{94}$ University of Wisconsin, Madison, WI, 
USA \\
$^{95}$ University of Wisconsin, Milwaukee, WI, 
USA \\
$^{96}$ Institute for Nuclear Science and Technology (INST), Hanoi, 
Vietnam \\
\par\noindent
(\ddag) Deceased \\
(a) at Konan University, Kobe, Japan \\
(b) now at the Universidad Autonoma de Chiapas on leave of absence from Cinvestav \\
(f) now at University of Maryland \\
(h) now at NYU Abu Dhabi \\
(i) now at Universit\'{e} de Lausanne \\
(j) at Station de Radioastronomie de Nan\c{c}ay, Observatoire de Paris, Nan\c{c}ay, France
% last updated: 5/7/2012 
\end{small}
\end{itshape}
% \end{center}
\end{flushleft}

